Resource Efficient Boolean Function Solver on Quantum Computer

Nonlinear boolean equation systems play an important role in a wide range of applications. Grover's algorithm is one of the best-known quantum search algorithms in solving the nonlinear boolean equation system on quantum computers. In this paper, we propose three novel techniques to improve the efficiency under Grover's algorithm framework. A W-cycle circuit construction introduces a recursive idea to increase the solvable number of boolean equations given a fixed number of qubits. Then, a greedy compression technique is proposed to reduce the oracle circuit depth. Finally, a randomized Grover's algorithm randomly chooses a subset of equations to form a random oracle every iteration, which further reduces the circuit depth and the number of ancilla qubits. Numerical results on boolean quadratic equations demonstrate the efficiency of the proposed techniques.

==> Makefile <==
name=main

all: $(name).pdf

$(name).pdf: $(name).tex $(name).bib qcircuit.sty
	pdflatex $(name)
	bibtex   $(name).aux
	pdflatex $(name)
	pdflatex $(name)

reply:
	pdflatex ReplyLetter
	pdflatex ReplyLetter

clean:
	rm -f $~ *.aux *.idx *.log *.blg *.toc *.dvi *.ps *.out *.gz *.bbl \
			 *.fdb_latexmk *.fls *.thm figure/*-eps-converted-to.pdf
cleanless:
	rm -f $~ *.aux *.idx *.log *.blg *.toc *.dvi *.ps *.out *.gz \
			 *.fdb_latexmk *.fls *.thm
cleanall:
	rm -f $~ *.aux *.idx *.log *.blg *.bbl *.toc *.dvi *.ps *.out *.gz \
			 *.fdb_latexmk *.fls *.thm \
	         figure/*-eps-converted-to.pdf $(name).pdf \
			 ReplyLetter.pdf
zip:
	zip $(name).zip *.sty *.bib *.bbl *.tex *.pdf figure/*.eps \
		figure/*.svg figure/*.pdf

